Security Assessment of Hierarchical Federated Deep Learning

Hierarchical federated learning (HFL) is a promising distributed deep learning model training paradigm, but it has crucial security concerns arising from adversarial attacks. This research investigates and assesses the security of HFL using a novel methodology by focusing on its resilience against adversarial attacks inference-time and training-time. Through a series of extensive experiments across diverse datasets and attack scenarios, we uncover that HFL demonstrates robustness against untargeted training-time attacks due to its hierarchical structure. However, targeted attacks, particularly backdoor attacks, exploit this architecture, especially when malicious clients are positioned in the overlapping coverage areas of edge servers. Consequently, HFL shows a dual nature in its resilience, showcasing its capability to recover from attacks thanks to its hierarchical aggregation that strengthens its suitability for adversarial training, thereby reinforcing its resistance against inference-time attacks. These insights underscore the necessity for balanced security strategies in HFL systems, leveraging their inherent strengths while effectively mitigating vulnerabilities.

==> extra.tex <==
\newpage

\appendix

\section{L-level FL algorithm} \label{algo} 

The details of the L-level FL procedure are presented in Algorithm \ref{algo:algo1} from section \ref{HFL_Model}.

\begin{algorithm}[h!]
    %\SetAlgoNoLine
    \footnotesize
    % \scriptsize 
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwBlock{DoParallel}{do in parallel}{end}
    %\SetKwBlock{foreach}{for each}
  
    % Set Function Names
    \SetKwFunction{FAggregation}{Aggregation}
    \SetKwFunction{FClientUpdate}{ClientUpdate}
    \SetKwProg{Fn}{Function}{:}{}

    \Input{
        ${D_n}$ - Dataset of client $n$ where $n \in N$
    }
    
    \Output{
       $w$ - weight vector of the global model
     }

     //{Run on client $n$}
     
     \Fn{\FClientUpdate{$w$}}{
        
        $\beta \gets$ (split $D_n$ into batches of size $B$)
        
        \uIf {client $n$ in the overlapping coverage areas} {
                wait until other training job finished.}
                
        \For {local epoch $e$ from $1$ to $|Ep|$} 
         {
         \ForEach {batch $b \in \beta$}
            {
               $w \gets w -  \eta  \Delta  F(w;b)$ 
            }
         }
        \KwRet $w$
     }


    //{Run on server $s$}
     
     \Fn{\FAggregation{$s_\ell$,$w_t$}}{

        \ForEach {round $t=1,2,\ldots,T_{\ell}$}{
            \uIf{$\ell= L-2$}{
                //{random set of clients}
                
                $C_{t}$ $\gets$ select randomly $C_p$ \% of clients from $A(s_\ell)$
                
                \textbf{foreach} {client $n \in C_{t}$}
                \DoParallel
                {
                    $w_{t+1}^{n}$ $\gets$ ClientUpdate($w_t$)
                    
                }
                $w_{t+1} \gets
                    \frac{\sum |D_n| . w_{t+1}^n}{\sum |D_n|}, {n \in R_t}$
            }
            \uElse {
                \textbf{foreach} {server $s_{\ell+1} \in A(s_\ell)$ } \DoParallel
                {
                    $w_{t+1}^{s_\ell} \gets$ Aggregation($s_{\ell+1}$,$w_t$)
                    
                }
                $w_{t+1} \gets
                    \frac{\sum |D_{s_\ell}| . w_{t+1}^{s_{\ell}}}{\sum|D_{s_\ell}|}$

            }
        }
        \KwRet $w_{t+1}$
     }

    //{Start federated learning}
    
    {$w_0 \gets$ initialise model's weight 
    
    $w \gets$  Aggregation($s_0$, $w_0$)}

\caption{L-level FedAvg}
\label{algo:algo1}
    
\end{algorithm}

\newpage

\section{Node Characteristics} \label{Node_char}

\subsection{Benign/malicious Client Characteristics:}
We consider a population of smart devices distributed across a city that implement image classification tasks. There exists a group of 100 clients that engage in communication with the server for the purpose of image classification model training. We assume that the client selected for participation remains constant throughout the training process. Every client trains a local classifier model to classify the images. For the client's local classifier model, we use both the simple and complex CNN architectures suggested by Zhou et al. in \cite{zhou2023toward}. Each client employs categorical crossentropy as their loss function and utilises the optimizer that implements the Adam algorithm to update their local model depending on the loss function. For the grayscale image dataset, the batch size was set to 32 and the number of epochs was set to 1. Whereas for the colour image datasets,the batch size was set to 64 and the number of epochs was set to 6. If a client is compromised, the client could act maliciously by implementing data poisoning (label flipping) or model poisoning (sign flipping). We evaluate the performance of the model while the number of malicious clients is 1, 5, and 10. We also evaluate the models when all of the malicious clients are located in the overlapping area of two regional edge servers. 

\subsection{Benign/malicious Server characteristics:}
There is one cloud server in each learning paradigm at level 0. The cloud server performs the FedAvg aggregation rule for 20 aggregation rounds. We assume that the cloud server is highly secure and has never been compromised during the learning process. On the other hand, edge servers in HFL have different characteristics. In 3L-HFL, there are 20 regional edge servers that are distributed at the same level and connected directly with the cloud server and directly with 5 clients in their coverage area. Each regional edge server performs the FedAvg aggregation rule for two aggregation rounds. The 4L-HFL has similar settings to the 3L-HFL; however, there are 4 edge servers distributed at the same level between the cloud server and the regional edge servers. Each edge server communicates with five regional edge servers and performs the FedAvg aggregation rule for three aggregation rounds. The total aggregation round of regional edge server is 40 and 120 rounds for 3L-HFL and 4L-HFL respectively. We assume that regional edge servers can be compromised and act maliciously by implementing model poisoning (sign flipping), whereas other edge servers are highly secure. We evaluate the performance of the model while the number of malicious servers is 1, 5, and 10.
\newpage

\section{Miscellaneous Tables} \label{tables}

\begin{itemize}

     \item The key notations used in this paper are summarised in Table \ref{tabel:key_notation} for section \ref{HFL_Model}.
     
    \item Table \ref{tab:attack_model} for section \ref{Attack_model} presents the attack models of inference-time attack and training-time attack with the methods we implement in this study.
   
\end{itemize}

\begin{table}
    \centering
    \caption{List of key notation}
    \begin{tabular}{cc}
       Symbol  & Description \\ \hline
       $|L|$ & Number of levels in the hierarchy\\
       $\ell$ & a level in the hierarchy where $\ell \in {0,1,\ldots,L}$\\ 
       $T_\ell$ & Number of aggregation rounds at level $\ell$\\
       $N$ & Set of clients \\
       $|N|$ & Number of clients\\
       $n$ & a client where $n \in N$\\
       $C_p$ & proportion of client participants \\
       $C_t$ & set of client participants selected at aggregation round $t$ \\
       $D_n$ & Dataset of client n where $n \in N$\\
       $|D_n|$ & number of sample in Dataset of client n where $n \in N$\\
       $S$ & Set of servers\\
       $|S|$ & Number of servers\\
       $s_\ell$ & a server at level $\ell$ where $s \in S$\\
       $s_0$ & the cloud server\\
       $s_{L-2}$ & a regional edge server at level $L-2$ communicate with clients\\
       $A(s_\ell)$ & set of nodes in coverage areas $A$ of server $s \in S$ at level $\ell$\\
       $|D_{s_\ell}|$ & number of sample in Dataset of all clients in $A(s_\ell)$ \\
       $|Ep|$ & number of epoch for client local training\\ 
       $B$ & Batch size for local training \\ 
       $\eta$ & Learning rate\\ \hline
    \end{tabular}
    \label{tabel:key_notation}
\end{table}

\begin{table}[t]
\centering
  \caption{Attack model}
  \label{tab:attack_model}
\begin{tabular}{lllll}
\hline
Attributes          & \multicolumn{4}{c}{Inference-time attack}                                                                                                                                                                                                                                                                \\ \hline
Attack methods     & \multicolumn{2}{l}{\begin{tabular}[l]{@{}l@{}}Adversarial   Patch(AP),\\ Fast Gradient Method(FGM),\\ Projected Gradient Descent(PGD), \\ Saliency Map Method(JSMA)\end{tabular}} & \multicolumn{2}{l}{\begin{tabular}[l]{@{}c@{}}Square Attack(SA), \\ Spatial Transformations Attack(ST)\end{tabular}} \\ \hline

Entry point        & \multicolumn{2}{l}{Client side}                                                                                                                                                   & \multicolumn{2}{l}{Client side}                                                                                      \\ 
Security violation & \multicolumn{2}{c}{Integrity}                                                                                                                                                     & \multicolumn{2}{c}{Integrity}                                                                                        \\ 
Attack Knowledge   & \multicolumn{2}{c}{White box}                                                                                                                                                     & \multicolumn{2}{c}{black box}                                                                                        \\ 
Access level       & \multicolumn{2}{c}{Test/inference Data}                                                                                                                                           & \multicolumn{2}{c}{Test/inference Data}                                                                              \\ 
Attack frequency   & \multicolumn{2}{c}{once at test time}                                                                                                                                             & \multicolumn{2}{c}{once at test time}                                                                                \\ 
\hline
Attribute          & \multicolumn{4}{c}{Training-time attack}                                                                                                                                                                                                                                                                 \\ \hline
Attack methods     & \begin{tabular}[c]{@{}c@{}}Targeted label flipping\\  with backdoor attack\end{tabular}       & \begin{tabular}[c]{@{}c@{}}Untargeted\\  label flipping attack\end{tabular}       & sign flipping                                             & sign flipping                                            \\ \hline

Entry point        & client-side                                                                                   & client-side                                                                       & client-side                                               & server-side                                              \\ 
Security violation & Integrity                                                                                     & Integrity                                                                         & Integrity                                                 & Integrity                                                \\ 
Attack Knowledge   & black box                                                                                     & black box                                                                         & White box                                                 & White box                                                \\ 
Access level       & Training data                                                                                 & Training data                                                                     & Model parameters                                          & Model parameters                                         \\ 
Attack frequency   & every round                                                                                   & every round                                                                       & every round                                               & every round                                              \\ 
 \hline
\end{tabular}
\end{table}

\newpage

\section{Miscellaneous Figures} \label{figures}

\begin{itemize}

     \item Figure \ref{fig:SystemModel} for section \ref{exp_des} illustrates the Experiment design.
      
     \item Figure \ref{fig:ITA-AT} for section \ref{AT} illustrates the improved MR of robust models (red solid line) achieved through adversarial training compared to vulnerable models (red dashed line). 
     
    \item Figure \ref{fig:TTA} for section \ref{TTA} depicts the consequences of training-time attack
   
\end{itemize}

\begin{figure}[!h]
\centering
\includegraphics[width=15cm]{Figures/SystemModel2.pdf}
\caption{Experiment design}
\label{fig:SystemModel}
\end{figure} 

